Fast KVzip: Efficient and Accurate LLM Inference with Gated KV Eviction

Efficient key-value (KV) cache management is crucial for the practical deployment of large language models (LLMs), yet existing compression techniques often incur a trade-off between performance degradation and computational overhead. We propose a novel gating-based KV cache eviction method for frozen-weight LLMs that achieves high compression ratios with negligible computational cost. Our approach introduces lightweight sink-attention gating modules to identify and retain critical KV pairs, and integrates seamlessly into both the prefill and decoding stages. The proposed gate training algorithm relies on forward passes of an LLM, avoiding expensive backpropagation, while achieving strong task generalization through a task-agnostic reconstruction objective. Extensive experiments across the Qwen2.5-1M, Qwen3, and Gemma3 families show that our method maintains near-lossless performance while evicting up to 70% of the KV cache. The results are consistent across a wide range of tasks, including long-context understanding, code comprehension, and mathematical reasoning, demonstrating the generality of our approach.

==> section/1-intro.tex <==
\section{Introduction}

Transformer-based LLMs have revolutionized the landscape of artificial intelligence, solving complex challenges ranging from long-context processing to advanced reasoning \citep{o1,gemini}.
A cornerstone of this success is the attention mechanism, which allows models to effectively contextualize features across sequences \citep{transformer}.
To mitigate the computational cost of re-calculating attention features at every step, inference systems adopt KV caching \citep{transformerxl}.

\begin{figure}[t]
    \centering
    \input{graph/intro}
    \vspace{-1em}
    \caption{\textbf{Highlighted results.} (a) Evaluation on the KVPress benchmark \citep{kvpress} (RULER-4K dataset, Qwen3-8B) compared to state-of-the-art methods from December 2025. (b) Chunked-prefill efficiency for 170K tokens using Qwen2.5-14B-1M with 30\% KV cache budget and BF16 precision.}
    \vspace{-0.5em}
    \label{graph:intro}
\end{figure}

However, the effectiveness of KV caching is increasingly strained by the growing demand for long-context inference. As the memory required to store KV features scales linearly with sequence length, KV caches become a dominant bottleneck during inference \citep{vllm}.
While KV cache eviction approaches alleviate this burden, they often face a critical dilemma: Methods with negligible compression overhead result in significant performance degradation \citep{h2o,snapkv}, while methods that preserve accuracy tend to incur prohibitive compression overhead \citep{kvzip}.
For instance, KVzip \citep{kvzip} relies on the reconstruction process that doubles computation during prefill (see \Crefsub{graph:intro}{b}), limiting its practicality for latency-sensitive deployment.

In this paper, we introduce \textbf{\textit{Fast KVzip}}, a fast and accurate KV cache eviction method that addresses the inefficiencies of prior reconstruction-based approaches.
Our key insight is that the future utilization of KV pairs is largely an \textit{intrinsic property} that can be directly decoded from the input hidden states, without reconstructing the entire context as in KVzip. Leveraging this insight, we seamlessly integrate a lightweight gating mechanism into the Transformer’s forward pass. This allows the model to directly assess the importance of KV pairs during both the prefill and decoding stages, incurring negligible memory and computational overhead while preserving high compression fidelity.

To identify an effective gating mechanism, we systematically explore the design space. Our empirical analysis reveals that gates perform most effectively when operating on input hidden states rather than intermediate attention features. Furthermore, we find that an architecture inspired by attention sinks \citep{streaming} yields the strongest performance.
Accordingly, we introduce a layer-wise gate training procedure that distills KV importance scores pre-computed from a compute-intensive reconstruction process. To ensure efficiency and avoid degrading the original model’s capabilities, we keep the LLM weights frozen and train only the gating parameters, requiring less than one H100 GPU hour for 14B-scale models.

As highlighted in \Cref{graph:intro}, Fast KVzip matches the compression performance of KVzip while maintaining model accuracy at KV budget ratios as low as 25\% on the RULER-4K benchmark \citep{ruler}, and significantly outperforms existing baselines on the KVPress benchmark (as of December 2025) \citep{kvpress}. Moreover, \Crefsub{graph:intro}{b} shows that Fast KVzip substantially reduces peak memory usage and prefill time compared to both KVzip and the no-compression baseline.

We further demonstrate the effectiveness and generality of our method across a diverse set of state-of-the-art open-source LLMs, including Qwen2.5-7B/14B-1M \citep{qwen}, Qwen3-8B/14B, Qwen3-8B-FP8 \citep{qwen3}, and Gemma3-12B \citep{gemma3}. Our approach is compatible with quantized weights and sliding-window hybrid attention mechanisms.
We evaluate on prefill-intensive long-context benchmarks such as SCBench \citep{scbench} and MRCR \citep{mrcr} with context lengths of up to 170K tokens, as well as decoding-intensive reasoning tasks including AIME24 \citep{aime} and MATH \citep{math}. Across all models and benchmarks, Fast KVzip achieves near-lossless performance while reducing the KV cache to 30$\minus$40\% of its original size, underscoring the robustness and practicality of the proposed gating-based eviction strategy.

==> section/2-background.tex <==
\begin{figure*}[t]
    \begin{center}
        \input{figure/method}
        \vspace{-0.5em}
        \caption{\textbf{Computational flow.} (a) Illustration of gating at each attention layer. (b) During each forward pass, we jointly calculate importance scores and evict low-importance KV pairs. For decoding, we maintain a small buffer to cache recent hidden states, performing gating and eviction in parallel once the buffer is full. This parallelized computation reduces latency overhead. We utilize a chunk size of 16K for prefill and a buffer size of 128 tokens for decoding; at each eviction step, we retain the KV pairs of the most recent tokens, keeping 4K tokens for prefill and 128 tokens for decoding.}
        \label{fig:method}
    \end{center}
\end{figure*}


\section{Related Work}
\paragraph{KV Cache Compression.}
To mitigate the scalability bottleneck of KV caching in autoregressive Transformers \citep{gpt2}, efficient attention mechanisms have been proposed, including sliding-window attention \citep{sparsetransformer}, linear attention \citep{linear}, latent attention \citep{mla}, and grouped-query attention \citep{gqa}. While effective, these methods typically require training from scratch or substantial fine-tuning to accommodate architectural changes.

Recent work observes inherent sparsity in LLM attention patterns \citep{dejavu}. Methods such as $\text{H}_2\text{O}$ \citep{h2o}, Finch \citep{corallo2024finch}, and SnapKV \citep{snapkv} exploit sparsity observed during prefill or decoding to evict under-utilized KV pairs. However, sparsity patterns inferred at inference time often overfit the current input and fail to generalize across future queries. To address this limitation, query-agnostic approaches, \textit{e.g.,} KVzip \citep{kvzip}, EpiCache \citep{epicache}, and Expected Attention \citep{kvpress}, estimate KV importance independently of specific queries and demonstrate improved robustness in multi-query settings. Orthogonal strategies, such as DuoAttention \citep{duo}, RLKV \citep{rlkv}, and FastGen \citep{fastgen}, predefine attention patterns (e.g., sliding-window or A-shaped) using calibration datasets prior to deployment. Beyond token-level eviction, complementary compression techniques explore alternative dimensions, including feature-channel compression \citep{think} and KV quantization \citep{kivi}.


\begin{table}[t]
    \centering
    \caption{\textbf{Gating strategies for Transformer attention.} The table below indicates operation execution per layer for a given input. Mixture-of-Depths (MoD) uses gating to skip attention computation, while Mixture-of-Block-Attention (MoBA) applies gating to select blocks for sparse attention with stored KV features. Our method bridges these approaches by conducting an attention operation for every input token while improving computational and memory efficiency through gated KV eviction.}
    \vspace{-0.2em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lll}
    \toprule
    Method & Attention & Store KV feature \\
    \midrule
    MoD \citep{mixture-depth} & Conditional  & Conditional \\
    MoBA \citep{moba} & Always & Always \\
    \midrule
    Fast KVzip (Ours) & Always & Conditional \\
    \bottomrule
    \end{tabular}    
    }
    \label{tab:gating_mechanism}
\end{table}


\paragraph{Gating in Transformers.}
To address the scaling issues of Transformers \citep{transformer}, researchers have introduced gating mechanisms that enable sparse and selective computation, including MoE \citep{moe}, MoD \citep{mixture-depth}, and MoBA \citep{moba}. These approaches demonstrate that pretraining with gating can effectively exploit sparsity in MLP and attention modules, improving computational efficiency. \Cref{tab:gating_mechanism} provides a conceptual comparison of these approaches with our method.

In the landscape of KV cache compression, Locret \citep{locret} employs a gating module to predict KV importance scores, while DMS \citep{dms} trains an eviction policy via logit distillation. Concurrent to our work, TrimKV \citep{trimkv} introduces a retention-gated mechanism to learn time-decaying importance scores.
Despite their promise, Locret is confined to prefill-stage compression, and TrimKV suffers from performance degradation in prefill-intensive scenarios, specializing in narrow domains of mathematical reasoning. In our work, we provide a comprehensive interpretation of the gating mechanism, demonstrating that well-designed gating architectures and optimization strategies achieve near-lossless compression across both prefill and decoding stages. We provide a more detailed comparison to prior methods in \Cref{appendix:experiment}.
We also note a concurrent work, KVzap \citep{kvzap}, which explores a similar gating optimization objective but differs in specific architecture and training recipe. Together with our work, these parallel efforts underscore the promise of gating-based approaches for KV cache compression.

==> section/3-method.tex <==
\section{Method}\label{sec:method}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gating Mechanism}

\paragraph{Formulation.} We design a gating module that processes the hidden features of each attention layer and outputs importance scores for the KV features in that layer. Specifically, the gate at layer $l$ is defined as
\begin{align*}
g_l: \mathbb{R}^D \rightarrow [0,1]^H,    
\end{align*}
where $D$ denotes the hidden feature dimension and $H$ is the number of KV heads in the layer. We introduce an additional gating branch into the model’s forward computation. This branch operates independently and does not affect the original attention outputs (see \Crefsub{fig:method}{a}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computational Flow.}

\Crefsub{fig:method}{b} illustrates the overall computational flow of our method. We adopt a chunked prefill to reduce the peak memory usage when processing long contexts \citep{prefill}. For each input chunk, we first compute the KV features and their corresponding importance scores using the gating mechanism. Based on these scores, we evict low-importance KV features from the cache, maintaining a compressed KV cache either at a fixed retention ratio or within a predefined memory budget. Our approach is compatible with both non-uniform and uniform KV cache structures \citep{adakv,snapkv}. Empirically, we observe that retaining KV features from recent tokens improves performance (see \Cref{appendix:exp_local_window}). By maintaining a compressed KV cache throughout chunked prefill, our method reduces the peak KV cache memory compared to naive chunked prefill, as shown in \Crefsub{graph:intro}{b}.

During decoding, we apply the same gated KV eviction strategy. However, computing gates at every decoding step introduces substantial overhead due to frequent function calls and increased I/O, resulting in a 30$\minus$60\% latency increase depending on the context length. To mitigate this issue, we maintain a small buffer of token length 128 that caches recent hidden states and periodically computes gating in parallel. After updating the importance scores, we perform KV compression accordingly. This strategy reduces the gating overhead to approximately 1\% of the model’s forward-pass latency on average.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interpretation of Gating Formulation}

\begin{figure}[t]
    \begin{center}
        \input{figure/baseline}
        \caption{\textbf{Gating formulation} of existing KV compression methods at each attention layer. Note that we compare the core components of baseline methods, as each method jointly uses other techniques. For instance, FastGen combines its approach with cumulative attention scores \citep{h2o}.
        }
        \label{fig:baseline}
    \end{center}
\end{figure}

Before detailing our method, we establish a conceptual basis for why gating mechanisms are effective for KV cache compression. Notably, we observe that several prominent compression methods can be reformulated as constrained instances of a generalized gating framework (\Cref{fig:baseline}).

For instance, DuoAttention \citep{duo} optimizes a head-level indicator function to designate specific heads for local-window attention. This represents a constrained gating formulation where the gating function is a constant Boolean mapping, independent of inputs. Expected Attention \citep{kvpress} approximates future attention scores by applying a quadratic model of key states with mean query-state statistics. Furthermore, FastGen \citep{fastgen} identifies heads that attend to specific token clusters (\textit{e.g.}, punctuation or special tokens), which can be interpreted as a head-wise gating function on input tokens.

Our gating approach generalizes these prior methods by allowing any differentiable gating function without imposing empirical and heuristic constraints on the optimization. This interpretation enables a principled approach to KV cache compression, transforming the problem from heuristic design to data-driven optimization, effectively utilizing the model to discover the optimal compression strategy.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Gate Training}\label{subsec:method_optimization}
\begin{figure}[t]
    \begin{center}
        \input{figure/optimization}
        \caption{\textbf{Gate training process.} We compute the importance scores of KV pairs for a given text input following KVzip, which calculates the maximum attention score each KV pair receives during the context reconstruction \citep{kvzip}. We train gating modules to predict these scores from the input hidden states at each attention layer. Please refer to \Cref{appendix:details} for further details and the training hyperparameters.}
        \label{fig:optimization}
    \end{center}
\end{figure}


\paragraph{Consideration.}
We impose three requirements on our optimization: (1) computational efficiency, (2) robustness to task-specific overfitting, and (3) preservation of the base LLM’s performance. End-to-end optimization via backpropagation, for example, incurs substantial memory overhead, limiting the usable context length and increasing training time. Furthermore, training gating mechanisms on data from a specific domain or task, such as mathematical reasoning \citep{trimkv} or instruction-based question answering \citep{locret}, may yield domain-specific gains but incur degraded performance on other domains or tasks.

\paragraph{Training Procedure.}
With these considerations, we propose a gate training procedure illustrated in \Cref{fig:optimization}. We optimize the gates at each layer using target scores derived from KVzip’s reconstruction process \citep{kvzip}, while freezing LLM weights to avoid altering the model’s inherent capabilities. This design is computationally efficient, as reconstruction can be performed using parallelized forward passes. Given the target scores, we optimize gates independently at each layer using stochastic gradient descent with a binary cross-entropy loss \citep{bce}. The resulting optimization is embarrassingly parallel across both samples and layers, enabling efficient GPU execution.

Reconstruction-based target signals have been shown to generalize well to downstream tasks \citep{bert,kvzip}, thereby mitigating task-overfitting issues. While KVzip introduces additional compression latency at inference time due to reconstruction, we perform this step only during a pre-deployment phase to train the gates. Consequently, inference remains fast. 

\paragraph{Training Data.} 
We train the gating mechanism using the FineWeb-Edu pretraining corpus \citep{fineweb}, which has no overlap with downstream evaluation datasets. We randomly sample sequences ranging from 10K to 30K tokens, yielding a total of 1M training tokens. Given that FineWeb-Edu contains over 1T tokens, our training set corresponds to approximately a $10^{-6}$ fraction of the full corpus.

\begin{figure}[t]
    \begin{center}
        \input{graph/opt-target}
        \vspace{-1em}
        \caption{\textbf{Effects of target scores} for gate training, derived from reconstruction, next-token prediction, and instruction-based QA tasks. We evaluate Qwen2.5-7B-1M on a synthetic key retrieval task from SCBench \citep{scbench} and the SQuAD QA task \citep{squad}.}
        \label{fig:opt-target}
    \end{center}
\end{figure}

\begin{figure}[t]
    \centering
    \input{figure/heatmap}
    \vspace{-1em}
    \caption{\textbf{Maximum attention scores} received by KV features across specific tasks. 
    We visualize layers 7, 14, and 21 of Qwen2.5-7B-1M, with other layers exhibiting similar patterns, using the gate training data from \Cref{fig:opt-target}.}
    \label{fig:heatmap}
\end{figure}

\begin{figure}[t]
    \begin{center}
        \input{graph/opt-input}
        \vspace{-1em}
        \caption{\textbf{Effects of gate inputs}, including hidden states, key states, and pre-RoPE key states, with the same settings as \Cref{fig:opt-target}.}
        \label{fig:opt-input}
    \end{center}
\end{figure}

 \paragraph{Alternatives.}
In \Cref{fig:opt-target}, we compare the reconstruction-based target KV scores with scores derived from next-token prediction \citep{trimkv} and instruction-based question answering \citep{locret}. We identically compute the maximum attention score received by each KV feature under each task. For instruction-based QA, we follow \citet{locret} and use the LongAlpaca dataset \citep{longalpaca}. \Cref{fig:opt-target} demonstrates that reconstruction-based targets generalize significantly better, while alternatives lead to inferior performance. 

\Cref{fig:heatmap} reveals that reconstruction-based attention patterns are uniform and structured across KV sequences. In contrast, next-token prediction generates denser patterns, reflecting more intensive feature contextualization. We hypothesize that the reconstruction task is effective because many downstream applications rely primarily on these high-level contextualized features \citep{kvzip}. To maintain necessary local dependencies, our method also preserves KV pairs within a sliding window (\Cref{fig:method}). Conversely, QA tasks exhibit sparse attention as they focus only on query-specific information. Consequently, gates trained solely on QA signals generalize poorly, failing to retain the sufficient information required for broader downstream tasks.

In \Cref{fig:opt-input}, we study the choice of gate inputs by comparing hidden states, key states, and pre-RoPE key states \citep{rope}. Hidden states consistently outperform the alternatives, indicating that they contain richer information for predicting the future utility of KV features. We also observe that incorporating position-encoded features degrades performance. This motivates decoupling positional information from the gating mechanism and instead leveraging recency through a simple local-window strategy (\Cref{fig:method}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Architecture}\label{subsec:architecture}

\paragraph{Consideration.} The primary objective in designing the gate architecture is to minimize computational and memory overhead while accurately modeling attention behavior to predict the future utilization of each KV feature.


\paragraph{Low-Rank Sink Attention.}
We introduce a lightweight, attention-inspired gating mechanism, illustrated in \Cref{fig:gate}. Given a hidden state $\mathbf{h}\in\mathbb{R}^D$, we apply linear projections followed by weighted normalization \citep{qwen3} to obtain $\mathbf{k}\in\mathbb{R}^{H\times D'}$ and $\mathbf{q}\in\mathbb{R}^{G\times H\times D'}$, where $H$ is the number of original KV heads and $G$ denotes the original grouped-query size \citep{gqa}. Both representations are low-dimensional relative to the original KV features.
The gate produces an importance score $\mathbf{s}\in\mathbb{R}^H$ via a sink-attention mechanism as
\begin{align*}
    \mathbf{s} = \frac{1}{G} \sum_{j=1}^G \frac{\text{exp}({\mathbf{q}_j}^\intercal\mathbf{k})}{\text{exp}({\mathbf{q}_j}^\intercal\mathbf{k})+ \underbrace{\sum_{r=1}^{S} \text{exp}({\mathbf{q}_j}^\intercal{\mathbf{k}_{\text{sink}}^{r}})}_{\text{Learnable sinks}}+b_j}.
\end{align*}
Here, $\mathbf{k}_{\text{sink}}^{r} \in \mathbb{R}^{H \times D'}$ are layer-specific learnable parameters that model sink keys, which play a critical role in standard attention mechanisms \citep{streaming}. We empirically observe that these features enable the gate to effectively estimate the importance of KV features for future attention. A scalar $b_j \ge 0$ serves as a bias controlling head-level importance. These parameters are trained jointly with the projection and normalization weights.

Unlike DeepSeek-V3.2, which employs a low-rank KV cache within its Lightning Indexer to enable sparse attention \citep{deepseekv3.2}, our method uses a fixed set of low-rank key features per layer and introduces no additional KV caching. This design simplifies implementation and enables straightforward integration into existing architectures.

Note that we use an identical set of hyperparameters across all models, setting $S=16$ and $D'=16$, which is $1/8$ of the Qwen3 head dimension \citep{qwen3}, which suggests that our method requires neither exhaustive hyperparameter search nor manual fine-tuning. We provide a sensitivity analysis of hyperparameters in \Cref{appendix:sensitivity}.


\begin{figure}[t]
    \begin{center}
        \input{figure/gate}
        \caption{\textbf{Gate architecture.} We propose a sink-attention architecture using a fixed set of keys per layer. Given a hidden state $\mathbf{h}\in\mathbb{R}^D$, we compute the importance scores of KV as $\mathbf{s}\in[0,1]^H$.}
        \label{fig:gate}
    \end{center}
\end{figure}


\begin{figure}[t]
    \begin{center}
        \input{graph/opt-architecture}
        \vspace{-1em}
        \caption{\textbf{Performance of gate architectures}. We compare our sink-attention, a variant without learnable denominator terms, a two-layer MLP, and a linear model, using Qwen2.5-7B-1M.}
        \label{fig:performance_architecture}
    \end{center}
\end{figure}


\paragraph{Alternatives.} 
We study alternative gate architectures, including a linear model, a two-layer MLP with SwiGLU activation \citep{swiglu}, and a variant of our architecture without a learnable denominator, \textit{i.e.,} setting $\sum_{r=1}^{S} \exp({\mathbf{q}_j}^\intercal{\mathbf{k}_{\text{sink}}^{r}}) + b_j = 1$. Except for the linear model, we match the parameter counts across all architectures.
\Cref{fig:performance_architecture} shows that while alternative architectures are competitive on contextual QA tasks, they exhibit degraded performance on retrieval tasks. These results highlight the effectiveness of our sink-attention gate architecture.

\begin{table}[t]
    \caption{\textbf{Training efficiency.} Gate training time and gate sizes across diverse model scales. The 30B-A3B model has a smaller hidden state size than the other models, resulting in smaller gates.}
    \centering
    \resizebox{\linewidth}{!}{%
    \small
    \begin{tabular}{lrr}
    \toprule
    Model    & \hspace{-1em}Training Time (H100 hours)  &  Storage (GB)  \\
    \midrule
    Qwen3-8B    & 0.59 & 0.18 \\
    Qwen3-30B-A3B  & 0.70  & 0.11 \\
    Qwen3-14B  &  0.83 & 0.30 \\
    \bottomrule
    \end{tabular}
    \label{tab:efficiency}
    }
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
  \begin{center}
    \input{graph/efficiency}
    \vspace{-1em}
    \caption{\textbf{Inference efficiency.} Prefill and decoding efficiency of the Qwen2.5-7B-1M model using a 30\% KV budget ratio with PyTorch and FlashAttention-2 \citep{flashattn} on a single H100 GPU. Points in the plot correspond to context lengths of 160K, 240K, and 320K.
    Note that KVzip provides a decoding speed similar to Fast KVzip, which is omitted from Figure (b) for clarity.}
    \label{fig:efficiency}
  \end{center}
\end{figure}


\begin{figure*}[t]
    \centering
    \input{graph/qwen2.5-7b}
    \vspace{-1.5em}
    \caption{\textbf{Prefill-intensive benchmark results} with Qwen2.5-7B-1M under varying KV cache budget ratios from 0.2 to 1.0. Tasks are organized into three categories: (1) retrieval-intensive, (2) contextual understanding, and (3) high context redundancy.}
    \label{graph:prefill_benchmark}
% \end{figure*}
% \begin{figure*}[t]
    \vspace{1.5em}
    \centering
    \input{graph/architecture}
    \vspace{-1.5em}
    \caption{\textbf{Performance across different models}, averaged over 12 benchmark datasets. For each dataset, results are normalized with respect to full-cache performance prior to averaging.}
    \label{graph:architecture}
\end{figure*}

\subsection{Efficiency}
\paragraph{Gate Training.} 
\Cref{tab:efficiency} shows the training time and memory requirements of our gate training process, demonstrating its efficiency across diverse model scales.

\paragraph{Inference.} \Cref{fig:efficiency} shows the memory and latency efficiency improvements of Fast KVzip during both prefill and decoding. The results demonstrate that Fast KVzip reduces latency and memory usage compared to the base model, while significantly improving prefilling efficiency compared to KVzip by removing the runtime KV cache compression overhead. For all experiments, we apply a non-uniform KV cache eviction structure following \citet{kvzip}.


==> section/4-experiment.tex <==



\section{Experiment}\label{sec:exp}

We evaluate the KV cache compression performance of Fast KVzip under both prefill-intensive and decoding-intensive scenarios. We train gates once per model using FineWeb-Edu \citep{fineweb} and evaluate on all downstream tasks (see \Cref{subsec:method_optimization}), demonstrating that the learned gates are task-generalizable. All gate training and model evaluations are conducted on a single NVIDIA H100 80GB GPU using PyTorch and FlashAttention-2 \citep{flashattn}.


\begin{figure*}[t]
  \begin{center}
    \input{graph/math}
    \vspace{-1.5em}
    \caption{\textbf{Decoding-intensive benchmark results}. For AIME24, we report the average score over 16 random seeds.}
    \label{graph:decoding_benchmark}
  \end{center}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup}

\paragraph{Datasets.}
For prefill-intensive scenarios, we evaluate all methods on SCBench \citep{scbench}, a multi-query benchmark comprising nine tasks, including synthetic key retrieval tasks from RULER \citep{ruler}, long-context question answering from LongBench \citep{longbench}, and code comprehension tasks. We further include OpenAI MRCR \citep{mrcr}, a multi-round conversational retrieval benchmark, and SQuAD \citep{squad}, a multi-query QA dataset.  The maximum context length reaches up to 170K tokens using the Qwen3 tokenizer.

For decoding-intensive tasks, we evaluate on mathematical reasoning benchmarks, AIME24 \citep{aime} and MATH \citep{math}. Following the R-KV baseline \citep{rkv}, we set the maximum decoding length to 32K tokens for AIME24 and 16K tokens for MATH.

\paragraph{Models.}
We conduct experiments on a diverse set of state-of-the-art open-source large language models, including Qwen2.5-7B/14B-1M \citep{qwen}, Qwen3-8B/14B, Qwen3-8B-FP8 \citep{qwen3}, and Gemma3-12B \citep{gemma3}. We evaluate each model using its native precision. Notably, Gemma3-12B employs a hybrid sliding-window attention mechanism, while Qwen3-8B-FP8 adopts dynamic FP8 quantization. For the hybrid model, we only compress the global attention KV cache, which dominates memory usage in long-context evaluation 

\paragraph{Baselines.}
We compare Fast KVzip against several state-of-the-art KV cache compression methods, including KVzip \citep{kvzip}, SnapKV \citep{snapkv}, Expected Attention \citep{kvpress} with Ada-KV \citep{adakv}, DuoAttention \citep{duo} with KVzip score \citep{kvzip}, R-KV \citep{rkv}, and TrimKV \citep{trimkv}. For prefill-intensive tasks, we evaluate methods under the query-agnostic setting, following the setting of KVzip \citep{kvzip}. 

For decoding-intensive tasks, we adopt the R-KV setting \citep{rkv}, which continuously compresses the KV cache during decoding, covering both the context and generated tokens, to match the fixed-size cache budget. Additionally, we evaluate the early stopping of thinking strategy introduced in Qwen3 \citep{qwen3}, where the model terminates the thinking process upon reaching a predefined budget and is forced to generate the final answer. Since some baselines are specifically designed for either prefill-intensive or decoding-intensive scenarios, we report comparisons only within their respective applicable settings.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Prefill-Intensive Tasks}

\Cref{graph:prefill_benchmark} shows the prefill KV cache compression performance across 12 datasets. The results demonstrate that Fast KVzip outperforms all baselines across all tasks while matching the performance of KVzip, which requires twice the prefilling computational cost for compression. The figure shows that Fast KVzip maintains full-cache performance at a 30$\minus$40\% KV cache budget ratio. On some tasks, Fast KVzip exhibits performance improvements, which we attribute to the denoising effect of attention induced by KV cache compression \citep{differential}.

\Cref{graph:architecture} presents the averaged relative performance across the 12 datasets for various LLMs, demonstrating that Fast KVzip maintains effectiveness across models with a different pre-/post-training (Qwen3-8B), a larger model scale (Qwen2.5-14B-1M), a different attention mechanism (Gemma3-12B), and a quantization (Qwen3-8B-FP8).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Decoding-Intensive Tasks}

\Cref{graph:decoding_benchmark} shows the KV cache compression performance on mathematical reasoning tasks, including AIME24 and MATH. The results demonstrate that Fast KVzip achieves superior performance compared to decoding-scenario compression baselines on Qwen3-8B and Qwen3-14B models. Fast KVzip achieves near-lossless performance with a KV budget size of 4K, whereas the early-stopping-of-thinking method drastically reduces reasoning performance. These results indicate that the model requires a sufficient length of thinking to deduce correct answers, and that Fast KVzip indeed maintains the necessary KV features for general inference, including reasoning procedures.


==> section/5-analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Qualitative Analysis}\label{sec:analysis}

We analyze the gating behavior of Qwen2.5-7B-1M using English book and code data from SCBench. \Cref{fig:heatmap-pred} illustrates the distribution of KV cache retention rates across attention heads under a total of 36\% KV cache budget. We observe that half of the heads (primarily in early layers) exhibit highly sparse KV caches, while the remaining heads show uniformly distributed retention rates. This suggests that the gates prioritize high-level features from middle-to-late layers over low-level features from early layers.

We categorize attention heads by their retention rates ($r$) into three types: sparse ($r<0.05$), medium ($0.05\le r<0.9$), and dense ($0.9\le r$). \Cref{tab:head_group} details the tokens most frequently evicted and retained by each head type. Notably, sparse heads predominantly retain tokens associated with punctuation or line-break tokens. In contrast, other heads tend to retain tokens that are frequent in the source data; these frequent tokens appear as both the most retained and most evicted in medium heads. We hypothesize that sparse heads capture high-level, summarized information \citep{punctuation}, indicating an attention pattern distinct from local-window mechanisms \citep{streaming}.



\begin{figure}[t]
  \begin{center}
    \vspace{-0.5em}
    \input{figure/heatmap-pred}
    \vspace{-1.5em}
    \caption{\textbf{Retention Rates per Attention Head.} We apply a 36\% KV cache budget to Qwen2.5-7B-1M, which has 28 layers with 4 KV heads per layer. The left side corresponds to the early layers.}
    \label{fig:heatmap-pred}
  \end{center}
\end{figure}


\begin{table}[t]
    \centering
    \caption{\textbf{Gate behavior analysis.} The most frequently retained and evicted tokens for each head type. The {\textbackslash}s represents a space.}
    \vspace{-0.2em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|r|r}
    \toprule
    Head Type & Most Retained (Top $1 \rightarrow 10$) & Most Evicted (Top $1 \rightarrow 10$)\\
    \midrule
    Sparse & . .{\textbackslash}n{\textbackslash}n .{\textbackslash}n , for :{\textbackslash}n {\textbackslash}n {\textbackslash}s all that& , the . and to of a I in was\\
    Medium & , . and the of to I in {\textbackslash}n a & the , and to of a . I in was \\
    Dense & , the . and to of a I in was & the {\textbackslash}s , a {\textbackslash}t {\textbackslash}s{\textbackslash}s ( 1 of I \\
    \bottomrule
    \end{tabular}    
    }
    \label{tab:head_group}
\end{table}

==> section/6-conclusion.tex <==
\section{Conclusion}
\paragraph{Summary.}
We propose Fast KVzip, a gating-based KV cache compression method that matches state-of-the-art performance while eliminating runtime compression overhead. Through principled analysis, we design an effective gating optimization and a lightweight sink-attention architecture. Extensive evaluations on both prefill- and decoding-intensive tasks show that Fast KVzip generalizes well across diverse downstream applications, including retrieval, code comprehension, and reasoning, reducing KV cache size to 30\% with negligible performance loss.

\paragraph{Limitations and Future Work.}
Prior gating methods for attention modules, such as MoD \citep{mixture-depth} and MoBA \citep{moba}, typically require from-scratch training to fit predefined structures. An important future direction is to study how applying our method during pretraining can induce hardware-efficient structured computation patterns. Moreover, exploring a unified framework that integrates these gating approaches is a promising avenue. In particular, the gating mechanism could be extended to support multi-choice decisions, including skipping computation, discarding KV features, or storing them for selective retrieval.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newpage
% \section*{Acknowledgements}

% \section*{Impact Statement}
% This paper aims to contribute to the advancement of the field of machine learning. While the work may have various potential societal implications, none are identified as requiring specific discussion in this context.

